Interpretable Image Clustering via Diffeomorphism-Aware K-Means

We design an interpretable clustering algorithm aware of the nonlinear structure of image manifolds. Our approach leverages the interpretability of $K$-means applied in the image space while addressing its clustering performance issues. Specifically, we develop a measure of similarity between images and centroids that encompasses a general class of deformations: diffeomorphisms, rendering the clustering invariant to them. Our work leverages the Thin-Plate Spline interpolation technique to efficiently learn diffeomorphisms best characterizing the image manifolds. Extensive numerical simulations show that our approach competes with state-of-the-art methods on various datasets.

==> old_pieces_of_text.tex <==
%With ubiquitous recording devices, the development of machine learning algorithms capable of analyzing data is required to provide a better understanding of complex interactions. A nowadays efficient approach to this goal is based on supervised algorithms. However, the cost and the potential requirement of an expert to produce the labels is often a substantial limitation. As such, from market segmentation to genomic sequence analysis, unsupervised algorithms remain crucial tools to elutriate strategies and knowledge \cite{dolnicar2003using,xu2010clustering}. A specific branch at the forefront of unsupervised learning, named clustering, aims at 
%organizing the data into groups based on distinct similarities.

%A specific branch of machine learning, known as clustering, aiming at organizing the data into groups based on distinct similarities, is often considered a bridge between supervised and unsupervised learning.

%In the realm of clustering algorithms, the development of proper metric space is critical \cite{he2013k,frey2002fast,990920}. The distance induced by this space allows the computation of similarity between the data as to assign them to the correct cluster. One of the pillars of clustering is the K-means algorithm \cite{macqueen1967some}. It is a commonly used clustering algorithm as it is efficient, simple, and interpretable. Based on a specific metric, the iterative computation of the distance between centroids and the dataset allows the estimation of clusters. 

%\\
%\\
%The problem of defining a distance between signals lying in high-dimensional space has often been a critical bottleneck toward high-performance clustering algorithms \cite{steinbach2004challenges}. Our approach to tackling this problem takes its roots on the work of \cite{pitts1947we} in the $40s$ which described how the networks underlying our vision is provided with a similarity detector that enable the detection of classes of equivalences \rom{I guess here, Yanis and Anirvan you might have something to say (maybe a better ref. or a better argument...)}. 

%Nowadays, the concept of invariance is commonly used for understanding and improving machine learning algorithms \cite{mallat2016understanding,bruna2013invariant,oyallon2017scaling,cohen2019gauge}.  

%When considering the visual appearance instead of the shape, two approaches have been mainly considered. The first one consists in the development of features that are invariant to specific transformations \cite{czaja2018scattering,charalampidis2005modified,bruna2013invariant,le2002unsupervised}. Performing the clustering in the feature space hardens the interpretability of the results and usually constrain the embedding method to be used to be invertible, as well as the difficulty of extracting these features reliably and consistently \cite{lim2004image}. 
%
%
%The other approach that is the central discussion in this paper considers the images as points in high-dimensional space, and one aims to capture the geometric relations between images in this space; these methods are called appearance manifold based approach and were introduced in \cite{262951} and successfully used to cluster images \cite{basri1998clustering,su2001modified,1211332}. 
%
%In this framework, several distances have been introduced considering the development of metric capturing the symmetry in the data \cite{fitzgibbon2002affine,simard2012transformation,lim2004image}. These were motivated by the fact that the Euclidean distance between two face images of different identities but with the same pose is always smaller than the Euclidean distance between two face images of the same individual but with a different pose. The aim of these distance is in fact to distinguish data based on their taxonomy and to be invariant to their orientations, position in the images, and illumination conditions. 
%
%While the direction has been pointed, the invariance captured by these metric is constrained to the affine case. However, signals are often subjected to more intricates and non-rigid symmetries that extend the affine transformations. For instance, even in the simple case of digit recognition, the hand-writing style of different persons cannot be simply represented by affine transformations. 
%
%Although the approaches mentioned above appear very general, the invariances captured by the proposed metrics are limited to the affine case. However, in practice, signals are more often subjected to more intricate and non-rigid symmetries, which cannot be accounted for by simple affine transformations. 
%
% For instance, in the famous case of hand-written digit recognition, the different writing styles cannot be simply represented by affine transformations.

%
%More generally, for every class of object, the transformation of its instances by  diffeomorphisms do not alter necessarily its identity. 
%In this work, we will consider that local diffeomorphisms have to be taken into account as to capture accurately the variance in the data, and therefore, the metric we develop will be invariant with respect to affine transformation as well as local diffeomorphisms. Such a metric provides robustness to the Affine Invariant K-means algorithm and improve drastically its accuracy. 

%variance in the data
%The mapping between two sets of landmarks is performed through an interpolation scheme. While being efficient and providing a framework capable of learning non-rigid transformations, i.e., altering the shape and size of a image, these techniques rely on landmarks, thus restraining the application for these efficient methods to specific applications. 
%we propose to introduce a hidden variable based model to learn the landmarks such that we can cast an image registration algorithm in our metric and alleviate the drawbacks of group theoretically based image transformation techniques.


%in the following 
%It is important to note that the linearity of the transformation in the coordinate space does not imply linearity in the image space. 
%

